Interweaving Multimodal Interaction with Flexible Unit Visualizations for Data Exploration

Multimodal interfaces that combine direct manipulation and natural language have shown great promise for data visualization. Such multimodal interfaces allow people to stay in the flow of their visual exploration by leveraging the strengths of one modality to complement the weaknesses of others. In this work, we introduce an approach that interweaves multimodal interaction combining direct manipulation and natural language with flexible unit visualizations. We employ the proposed approach in a proof-of-concept system, DataBreeze. Coupling pen, touch, and speech-based multimodal interaction with flexible unit visualizations, DataBreeze allows people to create and interact with both systematically bound (e.g., scatterplots, unit column charts) and manually customized views, enabling a novel visual data exploration experience. We describe our design process along with DataBreeze's interface and interactions, delineating specific aspects of the design that empower the synergistic use of multiple modalities. We also present a preliminary user study with DataBreeze, highlighting the data exploration patterns that participants employed. Finally, reflecting on our design process and preliminary user study, we discuss future research directions.

==> paper-structure.tex <==
1 Introduction
2 Related Work
    2.1 Post-WIMP and Multimodal Visualization Systems
    2.2 Unit Visualizations
3 Flexible Visual Data Exploration with Unit Visualizations
4 DataBreeze
    4.1 Design Considerations
    4.2 Usage Scenario: Exploring Colleges in the US
    4.3 Operations
    4.4 Pen & Touch Interactions
    4.5 Speech & Multimodal Interaction
        4.5.1 Processing User Utterances
        4.5.2 Managing Ambiguity
        4.5.3 Command Discovery and Feedback
5 Preliminary User Study
6 Results and Discussion
7 Limitations and Future Work
8 Conclusion



------------------------
1 Introduction
2 Related Work
    -- Post-WIMP (Intro of the RW)
    2.1 Multimodal Interaction for Visualization
        - clarify what we mean by "Multimodal Interaction"
    2.2 Unit Visualization (+Composite Physicalization)
3 Maximizing Synergy w/ Multimodal Interaction
    3.1 Hybrid & Flexible
    3.2 Motivating Scenario
    3.3 Goals
3 DataBreeze Design
    3.1 Multiomodal Interaction with Unit Visualization 
        - Motivating & Novel Usage Scenario (abstract level)
    3.2 Design Considerations/Goals
    3.3 Basic Operations
        - Design Rationale & Justification
        - Managing Ambiguity
4 DataBreeze
    - Proof-of-Concept system, realizing the design
    4.1 Interacting with DataBreeze
    4.2 Multimodal Interaction
        4.2.1 Three Types of Speech Commands
        4.2.2 Command Discovery and Feedback
5 Preliminary User Study
    5.x Results
6 Discussion & Future Work
    6.1 Observations
    6.2 Limitation 

==> sections/free-form-vde.tex <==
\section{Flexible Visual Data Exploration with Unit Visualizations}

Unit visualizations can be considered as digital equivalents of composite physicalizations~\cite{jansen2013interaction,le2019dynamic} that support reconfiguration of individual elements.
Le Goc et al.~\cite{le2019dynamic} identify \textit{level of actuation} (extent to which elements can rearrange themselves) and \textit{degree of manipulability} (extent to which its elements can be manually rearranged) as two key dimensions of composite physicalizations.
While these concepts are relevant to our work, we only focus on digital interfaces and hence, do not discuss explicitly discuss data physicalizations~\cite{jansen2015opportunities} in the remainder of this paper.
In the case of digital unit visualization systems, the two dimensions identified by Le Goc et al. can be equated to actions like specifying attributes to adjust visual encodings of data points (actuation) or directly manipulating data points to change their position or representation (manipulation).

By visually representing individual data cases, unit visualizations present a unique opportunity to support a high level of flexibility using both fully-actuated and fully-customized views, as well as hybrid views that combine the two (Figure~\ref{fig:flexibility-spectrum}).
For instance, by specifying a horizontal and vertical axis and assigning an attribute to each, one can create a scatterplot (an example of a fully-actuated view as shown in Figure~\ref{fig:flexibility-spectrum}A).
Alternatively, similar to arranging physical objects~\cite{huron2014constructing,le2019dynamic}, one could explicitly manipulate each data point to create a fully-customized view (Figure~\ref{fig:flexibility-spectrum}C).
And finally, combining both actuation and manipulation, one could manually create separate groups of points based on a specific criteria and then leverage the system to visualize the groups as independent scatterplots (Figure~\ref{fig:flexibility-spectrum}B).

This flexibility to switch between actuated and customized views can be a powerful tool during visual data exploration. 
For example, people can leverage well-known unit visualization layouts (e.g., scatterplots, unit column charts) to compare and correlate values.
Furthermore, once they identify a set of points they are interested in or have a specific criteria in mind (e.g., private colleges on the west coast with an average cost of under 30k), people can directly manipulate the visualization to explicitly position or color these points to create a customized view that best fits their mental model.
Unfortunately, supporting such flexible visual data exploration is challenging with current tools that primarily support interaction through direct manipulation and control panels or configuration menus~\cite{}.
While these are powerful and popular styles of interaction, they can be constraining (e.g. there may not be a one-to-one mapping between desired actions and the control panel options) and tedious (e.g. one may need to repeatedly move points and place them in specific locations) for creating hybrid or fully-customized views~\cite{}.

% Unfortunately, most existing tools do not support such flexible interaction, only allowing people to create fully-actuated views.
% One reason for this is that most current tools rely on control panels for specifying visualizations and this restricts the actions that can be performed to the fields provided in the control panel (e.g., setting X/Y axis, coloring by an attribute).
% Even in the tools that support direct manipulation of data points~\cite{}, user actions performed on a subset of points are typically propagated throughout the view and are not localized to the subset of points.
% For example, with ForceSPIRE or VisExemplar, when users adjust the position of points, the system recomputes the underlying layout resulting in an adjusted force-directed layout or a scatterplot/unit column chart, respectively.

Multimodal interfaces that combine direct manipulation (via pen/touch) and speech can provide robust support for flexible data exploration, allowing users to fluidly switch between actuated and customized views.
For instance, to create a scatterplot like in Figure~\ref{fig:flexibility-spectrum}A, one could say ``\textit{Visualize average cost and median debt}", use a menu to specify the X/Y axes, or speak out the attribute name while swiping horizontally/vertically.
Now to split this into two groups like in Figure~\ref{fig:flexibility-spectrum}B, one could select a desired set of points (e.g., points with \texttt{Average Cost>35k}) using pen/touch and repeat the same actions as in the first step.
However, because the actions were performed after selecting a set of points, the system can apply them locally only to the selected points.
Creating a view like in Figure~\ref{fig:flexibility-spectrum}C using direct manipulation alone would require users to perform the tedious actions of inspecting individual points and moving them into different groups.
Alternatively, with a multimodal interface, similar to Bolt's ``Put-That-There"~\cite{bolt1980put} one could simply point (with a finger/pen) and say ``\textit{Bring schools with average cost more than 35000 here}" to create the two groups.
One can then select individual groups to color them and finally write down what defines a group (in this case, values for the \textit{Average Cost} attribute) resulting in the customized view in Figure~\ref{fig:flexibility-spectrum}C.
